The TechQA Dataset

We introduce TechQA, a domain-adaptation question answering dataset for the technical support domain. The TechQA corpus highlights two real-world issues from the automated customer support domain. First, it contains actual questions posed by users on a technical forum, rather than questions generated specifically for a competition or a task. Second, it has a real-world size -- 600 training, 310 dev, and 490 evaluation question/answer pairs -- thus reflecting the cost of creating large labeled datasets with actual data. Consequently, TechQA is meant to stimulate research in domain adaptation rather than being a resource to build QA systems from scratch. The dataset was obtained by crawling the IBM Developer and IBM DeveloperWorks forums for questions with accepted answers that appear in a published IBM Technote---a technical document that addresses a specific technical issue. We also release a collection of the 801,998 publicly available Technotes as of April 4, 2019 as a companion resource that might be used for pretraining, to learn representations of the IT domain language.

==> corpus.tex <==
\section{The IBM Technote Corpus}
The IBM Technotes are a collection of technical documents that address specific information needs of customers.  They include canonical procedures to perform common tasks, such as upgrading software products, as well as official solutions to specific problems.  By design, Technotes have a focused scope and do not address broad classes of questions.
Also by design, Technotes are structured documents that follow templated layouts that depend on the type of information.  An exampoe is a Technote that describes how to upgrade a complex enterprise software installation.
\begin{itemize}
    \item What are Technotes
    \item What we provide in the corpus
    \item
\end{itemize}
